Newton correction methods for computing real eigenpairs of symmetric tensors

Real eigenpairs of symmetric tensors play an important role in multiple applications. In this paper we propose and analyze a fast iterative Newton-based method to compute real eigenpairs of symmetric tensors. We derive sufficient conditions for a real eigenpair to be a stable fixed point for our method, and prove that given a sufficiently close initial guess, the convergence rate is quadratic. Empirically, our method converges to a significantly larger number of eigenpairs compared to previously proposed iterative methods, and with enough random initializations typically finds all real eigenpairs. In particular, for a generic symmetric tensor, the sufficient conditions for local convergence of our Newton-based method hold simultaneously for all its real eigenpairs.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
%\usepackage{authblk}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{hhline}
\usepackage{multirow}
\usepackage {tikz}
\usepackage{bm}
\usetikzlibrary{calc, positioning, decorations.pathreplacing}
\usepackage{etoolbox}
\usepackage{todonotes}
\newcommand{\todoi}[1]{\todo[inline]{#1}}
\usepackage{mathtools}
\usepackage{autonum}
\usepackage{appendix}
%\mathtoolsset{showonlyrefs=true}

\makeatletter
\patchcmd{\@addmarginpar}{\ifodd\c@page}{\ifodd\c@page\@tempcnta\m@ne}{}{}
\makeatother
\reversemarginpar

\usetikzlibrary {positioning}
\definecolor {processblue}{cmyk}{0.96,0,0,0}
%\usepackage{amsmath,amssymb,amsthm,mathrsfs,amsfonts,dsfont}
\usepackage{amsmath,amssymb,amsfonts,dsfont,mathrsfs,environ}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Newton correction methods for computing real eigenpairs of symmetric tensors} 
\newcommand{\TheAuthors}{Ariel Jaffe, Roi Weiss, Boaz Nadler}

% Sets running headers as well as PDF title and authors
\headers{Newton methods for the symmetric tensor eigen-problem}{Ariel Jaffe, Roi Weiss, and Boaz Nadler}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Resubmitted to the editors, February 28, 2018.
\funding{This research was funded in part by the Intel
	Collaborative Research Institute for Computational
	Intelligence (ICRI-CI), and by NIH grant 1R01HG008383-01A1.}}}

% \Authors: full names plus addresses.
%\author[add1]{Ariel Jaffe} %\and Roi Weiss \and Boaz Nadler \thanks{Imagination Corp., Chicago, IL
%		(\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
%}
\author{
  Ariel Jaffe\thanks{Weizmann Institute of Science, Israel.
    Emails: \email{author's-first-name.last-name@weizmann.ac.il}.}
  \and
  Roi Weiss\footnotemark[2]
%  \thanks{Department of Applied Mathematics, Fictional    University, Boise, ID (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
  \and
  Boaz Nadler\footnotemark[2]
}
%\author{
%  Dianne Doe\thanks{Imagination Corp., Chicago, IL
%    (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
%  \and
%  Paul T. Frank\thanks{Department of Applied Mathematics, Fictional
%    University, Boise, ID (\email{ptfrank@fictional.edu},
%    \email{jesmith@fictional.edu}).}
%  \and
%  Jane E. Smith\footnotemark[3]
%}
%\author{Ariel Jaffe
%\and
%Roi Weiss
%\and Boaz Nadler\thanks{Weizmann Institute of Science, Israel}}
%\address[add1]{Department of Redundancy Department}
 
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator*{\argmin}{argmin}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclareMathOperator*{\argmax}{arg\!,max}
\newcommand{\T}{\mathcal T}
\newcommand{\C}{\mathcal C}
\newcommand{\R}{\mathbb R}
\newcommand{\A}{\mathbb A}
\newcommand{\Av}{\bm 1_{\mathbb A}}
\newcommand{\Avc}{\bm 1_{\mathbb A^c}}
%\DeclareMathOperator*{\H}{\mathcal H}
%\DeclareMathOperator*{\the}{\pmb \theta}
%\DeclareMathOperator*{\thk}{{\pmb\theta}^{(k)}}


\newcommand{\nrm}[1]{{\|#1\|}}
\newcommand{\eps}{\varepsilon}
\newcommand{\tDelta}{\tilde{\Delta}}

%% vector x
\newcommand{\xv}{\bm x}
\newcommand{\xk}{\bm x_{(k)}}
\newcommand{\xo}{\bm x_{(1)}}
\newcommand{\xz}{\bm x_{(0)}}
\newcommand{\xkpo}{\bm x_{(k+1)}}
\newcommand{\xast}{\bm x^\ast}
\newcommand{\yv}{\bm y}
\newcommand{\yz}{\bm y_{(0)}}
\newcommand{\yast}{\bm y^*}
\newcommand{\yastk}{\bm y_{(k)}^*}
\newcommand{\yk}{\bm y_{(k)}}
\newcommand{\ykpo}{\bm y_{(k+1)}}
\newcommand{\err}{e}
\newcommand{\lamk}{\lambda_{(k)}}
\newcommand{\lamz}{\lambda^{(0)}}
\newcommand{\lamast}{\lambda^\ast}
\newcommand{\g}{\gamma}
\newcommand{\bz}{\bm z}
\newcommand{\tA}{H}
\newcommand{\grad}{\bm g}
\newcommand{\bv}{\bm k}
\newcommand{\ortc}{\bm u}
\newcommand{\ortcast}{\ortc^*}
\newcommand{\im}{i_1,\ldots,i_m}
\newcommand{\xim}{x_{i_1}\ldots x_{i_m}}
\newcommand{\xlocal}{\xv_{\text{loc}}}

\newcommand{\beq}{\begin{eqnarray*}}
	\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
%\DeclareMathOperator*{\Dk}{\Delta^{(k)}}
%\DeclareMathOperator*{\Dast}{\Delta^\ast}
\NewEnviron{salign}{%
	\begin{align}\begin{split}
	\BODY
	\end{split}\end{align}
}
\renewcommand{\S}{\mathcal{S}}
%\newtheorem{definition}{Definition}
\graphicspath{{./figures/}}
\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

\newtheorem*{conjecture}{Conjecture}
\newtheorem{remark}{Remark}

